Speeding-up $q$-gram mining on grammar-based compressed texts

We present an efficient algorithm for calculating $q$-gram frequencies on strings represented in compressed form, namely, as a straight line program (SLP). Given an SLP $\mathcal{T}$ of size $n$ that represents string $T$, the algorithm computes the occurrence frequencies of all $q$-grams in $T$, by reducing the problem to the weighted $q$-gram frequencies problem on a trie-like structure of size $m = |T|-\mathit{dup}(q,\mathcal{T})$, where $\mathit{dup}(q,\mathcal{T})$ is a quantity that represents the amount of redundancy that the SLP captures with respect to $q$-grams. The reduced problem can be solved in linear time. Since $m = O(qn)$, the running time of our algorithm is $O(\min\{|T|-\mathit{dup}(q,\mathcal{T}),qn\})$, improving our previous $O(qn)$ algorithm when $q = \Omega(|T|/n)$.

==> table_fast_re.tex <==

\begin{tabular}{|c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
 \hline 

\multicolumn{16}{|c|}{XML} \\ \hline
& \multicolumn{5}{c|}{50MB} &  \multicolumn{5}{c|}{100MB} &  \multicolumn{5}{c|}{200MB} \\
& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{2,702,383}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{5,059,578}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{9,541,590}\\& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{0.67 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{1.40 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{2.95 secs}\\ \hline
$q$ & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA\\ \hline
2 & 5,314,589 & 5.6 & 8.9 & \textbf{1.6} & 1.8 & 9,990,573 & 11.3 & 19.2 & \textbf{3.3} & 3.7 & 18,889,991 & 22.9 & 41.7 & \textbf{6.7} & 7.6 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
3 & 9,937,868 & 12.5 & 8.9 & 3.4 & \textbf{2.6} & 18,873,282 & 26.4 & 19.3 & 6.8 & \textbf{5.3} & 35,997,477 & 55.7 & 41.7 & 13.4 & \textbf{10.9} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
4 & 13,626,992 & 19.7 & 8.9 & 7.0 & \textbf{3.4} & 26,148,183 & 42.8 & 19.3 & 14.1 & \textbf{7.1} & 50,436,835 & 93.3 & 41.8 & 28.6 & \textbf{14.5} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
5 & 16,756,976 & 26.7 & 8.9 & 11.9 & \textbf{4.0} & 32,376,812 & 58.1 & 19.3 & 24.3 & \textbf{8.5} & 63,059,637 & 129.3 & 41.7 & 49.1 & \textbf{17.4} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
6 & 19,491,702 & 32.7 & 9.0 & 17.5 & \textbf{4.6} & 37,864,370 & 71.8 & 19.3 & 35.3 & \textbf{9.8} & 74,281,125 & 158.7 & 41.7 & 71.7 & \textbf{20.1} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
7 & 21,885,130 & 36.9 & 8.9 & 22.1 & \textbf{5.1} & 42,698,489 & 81.9 & 19.4 & 45.1 & \textbf{10.7} & 84,335,787 & 181.1 & 41.7 & 93.7 & \textbf{21.9} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
8 & 24,014,909 & 41.0 & 8.9 & 26.4 & \textbf{5.5} & 47,010,310 & 90.2 & 19.4 & 54.7 & \textbf{11.6} & 93,314,211 & 198.3 & 41.9 & 113.1 & \textbf{24.0} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
9 & 25,785,959 & 45.6 & 9.0 & 30.6 & \textbf{5.7} & 50,623,774 & 98.4 & 19.4 & 63.1 & \textbf{12.1} & 101,299,977 & 218.9 & 41.6 & 130.7 & \textbf{25.1} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
10 & 27,446,978 & 48.8 & 9.0 & 33.7 & \textbf{5.9} & 53,904,652 & 107.2 & 19.3 & 69.8 & \textbf{12.5} & 108,357,402 & 235.7 & 41.8 & 147.7 & \textbf{26.5} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
25 & 43,226,953 & \textbf{0.0} & \textbf{0.0} & 93.3 & 9.5 & 86,067,829 & \textbf{0.0} & \textbf{0.0} & 201.3 & 20.7 & 175,170,902 & \textbf{0.0} & \textbf{0.0} & 446.6 & 45.1 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
50 & 53,026,890 & \textbf{0.0} & \textbf{0.0} & 138.9 & 11.6 & 105,157,043 & \textbf{0.0} & \textbf{0.0} & 297.3 & 24.7 & 212,482,465 & \textbf{0.0} & \textbf{0.0} & 665.4 & 54.0 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
75 & 54,111,027 & \textbf{0.0} & \textbf{0.0} & 165.7 & 12.0 & 107,763,702 & \textbf{0.0} & \textbf{0.0} & 354.1 & 26.1 & 224,793,547 & \textbf{0.0} & \textbf{0.0} & 783.9 & 58.5 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
100 & 58,767,914 & \textbf{0.0} & \textbf{0.0} & 193.5 & 12.8 & 116,547,129 & \textbf{0.0} & \textbf{0.0} & 407.9 & 27.7 & 234,532,163 & \textbf{0.0} & \textbf{0.0} & 866.1 & 60.2 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
 \hline \hline
\multicolumn{16}{|c|}{DNA} \\ \hline
& \multicolumn{5}{c|}{50MB} &  \multicolumn{5}{c|}{100MB} &  \multicolumn{5}{c|}{200MB} \\
& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{6,406,324}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{12,233,978}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{23,171,463}\\& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{0.72 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{1.51 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{3.18 secs}\\ \hline
$q$ & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA\\ \hline
2 & 12,812,066 & \textbf{2.0} & 12.5 & 3.1 & 5.0 & 24,467,307 & \textbf{4.1} & 27.5 & 6.4 & 10.8 & 46,341,894 & \textbf{8.6} & 61.7 & 13.0 & 22.7 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
3 & 25,605,972 & \textbf{3.8} & 12.4 & 4.9 & 7.1 & 48,911,992 & \textbf{7.9} & 27.3 & $\triangleright 9.4$  & 14.8 & 92,653,730 & \textbf{16.4} & 61.7 & $\triangleright 19.1$  & 31.1 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
4 & 38,156,623 & \textbf{6.0} & 12.5 & 7.5 & 9.6 & 73,046,330 & \textbf{12.7} & 27.4 & 15.3 & 20.3 & 138,554,446 & \textbf{26.4} & 61.4 & 30.5 & 41.7 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
5 & 49,580,495 & \textbf{8.3} & 12.4 & 11.3 & 12.8 & 95,538,489 & \textbf{17.4} & 27.3 & 22.4 & 26.5 & 182,115,218 & \textbf{36.2} & 61.4 & 45.3 & 54.2 \\
\cline{1-1} \wcline{2-6} \wcline{7-11} \wcline{12-16}
6 & 58,545,479 & \textbf{10.8} & 12.4 & 15.8 & 16.1 & 114,077,582 & \textbf{22.1} & 27.4 & 31.3 & 33.0 & 219,484,022 & \textbf{46.2} & 61.7 & 63.4 & 68.6 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
7 & 62,855,357 & 15.0 & \textbf{12.4} & 21.7 & 18.8 & 124,372,705 & 30.6 & \textbf{27.3} & 43.5 & 39.4 & 242,809,754 & 62.3 & \textbf{61.4} & 86.9 & 82.9 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
8 & 63,209,540 & 20.5 & \textbf{12.4} & 28.5 & 20.2 & 126,873,871 & 41.0 & \textbf{27.5} & 58.0 & 43.2 & 251,230,926 & 83.4 & \textbf{61.7} & 115.0 & 93.5 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
9 & 61,361,180 & 28.9 & \textbf{12.4} & 38.0 & 20.4 & 124,483,208 & 57.3 & \textbf{27.5} & 77.2 & 44.4 & 249,275,546 & 116.1 & \textbf{61.2} & 154.9 & 96.1 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
10 & 58,962,119 & 49.5 & \textbf{12.4} & 59.6 & 19.9 & 120,367,281 & 98.5 & \textbf{27.4} & 119.4 & 43.9 & 243,013,084 & 199.8 & \textbf{61.5} & 241.9 & 96.3 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
25 & 52,805,704 & \textbf{0.0} & \textbf{0.0} & 193.0 & 17.2 & 105,798,123 & \textbf{0.0} & \textbf{0.0} & 434.2 & 37.5 & 211,410,696 & \textbf{0.0} & \textbf{0.0} & 957.1 & 82.0 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
50 & 52,250,573 & \textbf{0.0} & \textbf{0.0} & 196.6 & 16.1 & 104,722,871 & \textbf{0.0} & \textbf{0.0} & 445.3 & 35.1 & 209,263,031 & \textbf{0.0} & \textbf{0.0} & 981.4 & 78.0 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
75 & 52,186,606 & \textbf{0.0} & \textbf{0.0} & 198.4 & 15.9 & 104,529,341 & \textbf{0.0} & \textbf{0.0} & 445.2 & 34.6 & 208,812,015 & \textbf{0.0} & \textbf{0.0} & 989.3 & 76.3 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
100 & 52,167,349 & \textbf{0.0} & \textbf{0.0} & 198.8 & 15.7 & 104,490,733 & \textbf{0.0} & \textbf{0.0} & 443.7 & 34.5 & 208,662,988 & \textbf{0.0} & \textbf{0.0} & 985.6 & 75.9 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
 \hline \hline
\multicolumn{16}{|c|}{ENGLISH} \\ \hline
& \multicolumn{5}{c|}{50MB} &  \multicolumn{5}{c|}{100MB} &  \multicolumn{5}{c|}{200MB} \\
& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{4,861,619}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{10,063,953}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{18,945,126}\\& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{0.82 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{1.75 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{3.74 secs}\\ \hline
$q$ & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA\\ \hline
2 & 9,653,431 & 5.1 & 11.7 & \textbf{2.9} & 3.7 & 20,015,008 & 10.5 & 25.6 & \textbf{6.6} & 9.0 & 37,728,883 & 21.5 & 56.8 & \textbf{13.3} & 19.2 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
3 & 18,868,334 & 10.9 & 11.8 & 5.9 & \textbf{5.4} & 39,293,581 & 23.1 & 25.6 & 13.0 & \textbf{12.5} & 74,403,810 & 48.5 & 56.6 & 25.7 & \textbf{25.6} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
4 & 27,025,662 & 18.7 & 11.7 & 12.9 & \textbf{7.6} & 56,692,480 & 40.0 & 25.6 & 28.7 & \textbf{17.3} & 108,169,541 & 84.8 & 57.0 & 56.2 & \textbf{35.0} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
5 & 33,737,343 & 29.0 & 11.7 & 26.3 & \textbf{9.9} & 71,453,705 & 63.7 & 25.6 & 58.2 & \textbf{22.5} & 137,663,240 & 137.4 & 56.6 & 114.9 & \textbf{45.2} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
6 & 38,711,390 & 43.0 & 11.8 & 43.8 & \textbf{11.7} & 82,878,846 & 95.0 & \textbf{25.6} & 99.9 & $\triangleright 26.9$  & 161,235,051 & 205.9 & 56.4 & 198.4 & \textbf{55.3} \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
7 & 42,087,049 & 57.4 & \textbf{11.8} & 61.7 & 13.1 & 91,022,179 & 127.2 & \textbf{25.8} & 144.1 & 30.2 & 178,835,224 & 276.4 & \textbf{56.7} & 291.8 & 63.4 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
8 & 43,833,977 & 71.0 & \textbf{11.7} & 78.3 & 14.0 & 95,796,176 & 156.8 & \textbf{25.8} & 183.0 & 32.8 & 190,155,947 & 341.7 & \textbf{56.6} & 376.7 & 69.7 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
9 & 44,499,850 & 83.2 & \textbf{11.9} & 90.6 & 14.4 & 98,046,572 & 185.8 & \textbf{25.9} & 216.9 & 34.0 & 196,202,748 & 405.6 & \textbf{57.3} & 455.8 & 73.6 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
10 & 44,255,268 & 95.5 & \textbf{11.9} & 100.6 & 14.6 & 98,142,257 & 213.9 & \textbf{25.9} & 244.3 & 34.8 & 197,774,509 & 469.4 & \textbf{57.4} & 524.6 & 75.7 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
25 & 38,591,885 & \textbf{0.0} & \textbf{0.0} & 117.6 & 11.9 & 83,827,564 & \textbf{0.0} & \textbf{0.0} & 289.8 & 28.4 & 167,532,263 & \textbf{0.0} & \textbf{0.0} & 648.2 & 62.4 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
50 & 38,972,831 & \textbf{0.0} & \textbf{0.0} & 121.5 & 11.3 & 84,294,334 & \textbf{0.0} & \textbf{0.0} & 295.3 & 26.9 & 167,920,014 & \textbf{0.0} & \textbf{0.0} & 659.2 & 57.9 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
75 & 39,321,107 & \textbf{0.0} & \textbf{0.0} & 122.8 & 11.2 & 84,868,126 & \textbf{0.0} & \textbf{0.0} & 299.2 & 26.5 & 168,758,723 & \textbf{0.0} & \textbf{0.0} & 665.2 & 57.3 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
100 & 39,577,569 & \textbf{0.0} & \textbf{0.0} & 124.1 & 11.1 & 85,184,799 & \textbf{0.0} & \textbf{0.0} & 301.3 & 26.3 & 169,397,077 & \textbf{0.0} & \textbf{0.0} & 668.2 & 56.9 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
 \hline \hline
\multicolumn{16}{|c|}{PROTEINS} \\ \hline
& \multicolumn{5}{c|}{50MB} &  \multicolumn{5}{c|}{100MB} &  \multicolumn{5}{c|}{200MB} \\
& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{10,357,053}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{18,806,316}& \multicolumn{3}{r}{SLP Size:} & \multicolumn{2}{r|}{32,375,988}\\& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{0.82 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{1.75 secs}& \multicolumn{3}{r}{decompression time:} & \multicolumn{2}{r|}{3.74 secs}\\ \hline
$q$ & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA & \multicolumn{1}{c|}{$|z|$} & NMP & NSA & SMP & SSA\\ \hline
2 & 20,679,811 & \textbf{4.2} & 12.9 & 6.2 & 8.4 & 37,578,401 & \textbf{8.4} & 28.7 & 12.0 & 16.3 & 64,698,832 & \textbf{16.8} & 60.6 & 21.6 & 30.7 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
3 & 38,399,478 & \textbf{9.0} & 12.9 & 11.9 & 14.3 & 70,769,098 & \textbf{18.0} & 28.8 & 22.6 & 28.1 & 123,181,575 & \textbf{36.2} & 60.8 & $\triangleright 39.7$  & 50.6 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
4 & 46,663,331 & 20.5 & \textbf{12.9} & 24.4 & 19.7 & 88,478,549 & 40.8 & \textbf{28.7} & 45.9 & 39.0 & 156,086,678 & 82.2 & \textbf{60.8} & 81.1 & 73.5 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
5 & 43,546,201 & 59.7 & \textbf{12.9} & 59.6 & 20.3 & 83,931,339 & 123.1 & \textbf{28.7} & 116.4 & 41.7 & 151,179,701 & 241.5 & \textbf{60.6} & 208.5 & 79.1 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
6 & 40,978,356 & 104.7 & \textbf{13.1} & 101.9 & 19.2 & 78,814,777 & 223.0 & \textbf{28.9} & 200.9 & 39.9 & 142,407,894 & 444.4 & \textbf{61.0} & 363.7 & 75.8 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
7 & 40,609,196 & 128.3 & \textbf{13.0} & 124.2 & 18.5 & 77,777,885 & 287.0 & \textbf{29.1} & 258.1 & 38.2 & 140,157,823 & 593.4 & \textbf{61.0} & 491.4 & 72.6 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
8 & 40,841,595 & 133.0 & \textbf{13.0} & 128.1 & 18.1 & 78,209,687 & 301.6 & \textbf{28.9} & 272.8 & 37.4 & 140,969,562 & 627.1 & \textbf{60.9} & 525.4 & 71.1 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
9 & 41,173,093 & 134.7 & \textbf{13.0} & 129.4 & 17.7 & 78,931,535 & 307.0 & \textbf{28.9} & 274.0 & 36.6 & 142,587,195 & 637.1 & \textbf{61.2} & 535.0 & 69.9 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
10 & 41,489,300 & 135.8 & \textbf{12.9} & 130.3 & 17.4 & 79,662,935 & 309.3 & \textbf{28.8} & 279.3 & 36.3 & 144,220,125 & 649.6 & \textbf{61.2} & 538.0 & 69.3 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
25 & 44,337,428 & \textbf{0.0} & \textbf{0.0} & 139.2 & 16.1 & 86,053,654 & \textbf{0.0} & \textbf{0.0} & 302.3 & 34.0 & 159,309,786 & \textbf{0.0} & \textbf{0.0} & 595.4 & 65.4 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
50 & 46,641,113 & \textbf{0.0} & \textbf{0.0} & 146.5 & 15.9 & 91,434,913 & \textbf{0.0} & \textbf{0.0} & 326.0 & 33.9 & 172,456,054 & \textbf{0.0} & \textbf{0.0} & 651.3 & 66.4 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
75 & 48,127,663 & \textbf{0.0} & \textbf{0.0} & 154.2 & 16.0 & 94,859,488 & \textbf{0.0} & \textbf{0.0} & 342.0 & 34.6 & 180,871,898 & \textbf{0.0} & \textbf{0.0} & 691.3 & 68.9 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}
100 & 49,211,518 & \textbf{0.0} & \textbf{0.0} & 159.9 & 16.2 & 97,273,724 & \textbf{0.0} & \textbf{0.0} & 357.0 & 34.9 & 186,972,171 & \textbf{0.0} & \textbf{0.0} & 734.0 & 69.9 \\
\cline{1-1} \cline{2-6} \cline{7-11} \cline{12-16}

\end{tabular}


